The Blacklisting Memory Scheduler: Balancing Performance, Fairness and Complexity

In a multicore system, applications running on different cores interfere at main memory. This inter-application interference degrades overall system performance and unfairly slows down applications. Prior works have developed application-aware memory schedulers to tackle this problem. State-of-the-art application-aware memory schedulers prioritize requests of applications that are vulnerable to interference, by ranking individual applications based on their memory access characteristics and enforcing a total rank order. In this paper, we observe that state-of-the-art application-aware memory schedulers have two major shortcomings. First, such schedulers trade off hardware complexity in order to achieve high performance or fairness, since ranking applications with a total order leads to high hardware complexity. Second, ranking can unfairly slow down applications that are at the bottom of the ranking stack. To overcome these shortcomings, we propose the Blacklisting Memory Scheduler (BLISS), which achieves high system performance and fairness while incurring low hardware complexity, based on two observations. First, we find that, to mitigate interference, it is sufficient to separate applications into only two groups. Second, we show that this grouping can be efficiently performed by simply counting the number of consecutive requests served from each application. We evaluate BLISS across a wide variety of workloads/system configurations and compare its performance and hardware complexity, with five state-of-the-art memory schedulers. Our evaluations show that BLISS achieves 5% better system performance and 25% better fairness than the best-performing previous scheduler while greatly reducing critical path latency and hardware area cost of the memory scheduler (by 79% and 43%, respectively), thereby achieving a good trade-off between performance, fairness and hardware complexity.

==> tables/interval-sensitivity.tex <==
\footnotesize{
\begin{tabular}{|c|c|c|c|c|c|}
  \hline
  {Interval Length} & 1000 & 10000 & 100000\\
  \hline 
  {Weighted Speedup} & 1.10 &  1.18 & 1.10\\
  \hline 
  {Maximum Slowdown} &  0.73 & 0.79 &  0.84\\
  \hline 
\end{tabular}
}


==> tables/shared-caches.tex <==
\begin{tabular}{|c|c|c|c|}
    \hline
    Metric & FRFCFS & TCM & BLISS\\
    \hline
    Weighted Speedup (Normalized) & 1 & 1.13 & 1.18\\
    \hline
    Maximum Slowdown (Normalized) & 1 & 0.99 & 0.75\\
    \hline
\end{tabular}


==> tables/threshold-sensitivity.tex <==
\footnotesize{
\begin{tabular}{|c|c|c|c|c|c|}
  \hline
  {Blacklisting Threshold} & 2 & 4 & 8 & 16\\
  \hline
  {Weighted Speedup} & 1.11 & 1.18 &  1.16 & 1.10\\
  \hline
  {Maximum Slowdown} & 0.75 & 0.79 &  0.89 & 0.75\\
  \hline 
\end{tabular}
}

